SoK: Decentralized Finance (DeFi) Attacks

Within just four years, the blockchain-based Decentralized Finance (DeFi) ecosystem has accumulated a peak total value locked (TVL) of more than 253 billion USD. This surge in DeFi's popularity has, unfortunately, been accompanied by many impactful incidents. According to our data, users, liquidity providers, speculators, and protocol operators suffered a total loss of at least 3.24 billion USD from Apr 30, 2018 to Apr 30, 2022. Given the blockchain's transparency and increasing incident frequency, two questions arise: How can we systematically measure, evaluate, and compare DeFi incidents? How can we learn from past attacks to strengthen DeFi security? In this paper, we introduce a common reference frame to systematically evaluate and compare DeFi incidents, including both attacks and accidents. We investigate 77 academic papers, 30 audit reports, and 181 real-world incidents. Our data reveals several gaps between academia and the practitioners' community. For example, few academic papers address "price oracle attacks" and "permissonless interactions", while our data suggests that they are the two most frequent incident types (15% and 10.5% correspondingly). We also investigate potential defenses, and find that: (i) 103 (56%) of the attacks are not executed atomically, granting a rescue time frame for defenders; (ii) SoTA bytecode similarity analysis can at least detect 31 vulnerable/23 adversarial contracts; and (iii) 33 (15.3%) of the adversaries leak potentially identifiable information by interacting with centralized exchanges.

==> incidents.tex <==
\newcolumntype{L}{@{\extracolsep{2pt}}l@{\extracolsep{0pt}}}%
\newcolumntype{C}{@{\extracolsep{2pt}}c@{\extracolsep{0pt}}}%
\newcolumntype{v}{@{\extracolsep{6pt}}c@{}}%
\newcolumntype{v}{@{\extracolsep{6pt}}c@{}}%

\afterpage{%
\begin{landscape}
\begin{table}
\setlength{\tabcolsep}{0pt}
\centering
\caption{DeFi incidents taxonomy. We label the incident types that each academic paper and auditing report address. We also group the incidents that occur in the wild. Despite that this table focuses on Ethereum and BSC, we anticipate the taxonomy remains generic and thus applicable to all DeFi enabled blockchains. \ding{108}~-~Incident type addressed; \ding{110}~-~Incident type checked (likely with tools); \ding{111}~-~Incident cause checked (likely with tools); \ding{109}~-~Incident type checked (manually). Note that we can only be sure that an incident type has been addressed if an auditing report: (i) explicitly warns of the risk of a potential incident, or (ii) explicitly states that the code passed the check of an incident type.}
\label{table:cause_taxonomy}
\resizebox{1.29\textwidth}{!}{

\begin{tabular}{LLL Ccccccc Ccccccccccccccccccccccccccccc Cccccccccccccccccccccccccccccccccccccccccc Ccccc Ccccc Cccc Ccccc Ccccc Cccccc Ccc}
\toprule
& & &\multicolumn{78}{c}{Academic Papers} & \multicolumn{30}{c}{Audit Reports} & \multicolumn{3}{c}{Stats} \\
& & &\multicolumn{7}{c}{SoKs and Surveys} & \multicolumn{29}{c}{Tools} & \multicolumn{42}{c}{Papers} & \multicolumn{5}{c}{Boesin} & \multicolumn{5}{c}{PeckShield} & \multicolumn{4}{c}{SlowMist} & \multicolumn{5}{c}{Consensys} & \multicolumn{5}{c}{Certik} & \multicolumn{6}{c}{Trail of Bits} & \\




 &  &  & \rot[90]{\cite{praitheeshan2019security}} & \rot[90]{\cite{homoliak2020security}} & \rot[90]{\cite{saad2019exploring}} & \rot[90]{\cite{chen2020survey}} & \rot[90]{\cite{werner2021sok}} & \rot[90]{\cite{atzei2017survey}} & \rot[90]{\cite{samreen2021survey}} & \rot[90]{\cite{so2021smartest}USENIX'21 (SMARTEST)} & \rot[90]{\cite{zhang2020txspector}USENIX'20 (TxSpector)} & \rot[90]{\cite{zhou2020ever}USENIX'20} & \rot[90]{\cite{krupp2018teether}USENIX'18 (teether)} & \rot[90]{\cite{bose2022sailfish}SSP'22 (Sailfish)} & \rot[90]{\cite{zhou2021just}SSP'21 (DeFiPoser)} & \rot[90]{\cite{nguyen2021sguard}SSP'21 (SGUARD)} & \rot[90]{\cite{stephens2021smartpulse}SSP'21 (SmartPulse)} & \rot[90]{\cite{permenev2020verx}SSP'20 (Verx)} & \rot[90]{\cite{so2020verismart}SSP'20 (VeriSmart)} & \rot[90]{\cite{schneidewind2020ethor}CCS'20 (ethor)} & \rot[90]{\cite{he2019learning}CCS'19} & \rot[90]{\cite{tsankov2018securify}CCS'18 (Securify)} & \rot[90]{\cite{hou2019squirrl}NDSS'21 (SquirRL)} & \rot[90]{\cite{chen2020soda}NDSS'20 (SODA)} & \rot[90]{\cite{rodler2018sereum}NDSS'19 (Sereum)} & \rot[90]{\cite{kalra2018zeus}NDSS'18 (Zeus)} & \rot[90]{\cite{nguyen2020sfuzz}ICSE'20 (sFuzz)} & \rot[90]{\cite{grech2019gigahorse}ICSE'19 (Gigahorse)} & \rot[90]{\cite{choi2021smartian}ASE'21 (SMARTIAN)} & \rot[90]{\cite{feng2020summary}ASE'20} & \rot[90]{\cite{jiang2018contractfuzzer}ASE'18 (ContractFuzzer)} & \rot[90]{\cite{liu2018s}ASE'18 (Sgram)} & \rot[90]{\cite{luu2016making} (Oyente)} & \rot[90]{\cite{brent2018vandal} (Vandal)} & \rot[90]{\cite{albert2018ethir} (Ethir)} & \rot[90]{\cite{nikolic2018finding} (MAIAN)} & \rot[90]{\cite{wu2021defiranger}} & \rot[90]{\cite{chen2017under}} & \rot[90]{\cite{su2021evil}USENIX'21} & \rot[90]{\cite{perez2021smart}USENIX'21} & \rot[90]{\cite{torres2021frontrunner}USENIX'21} & \rot[90]{\cite{szalachowski2019strongchain}USENIX'19} & \rot[90]{\cite{torres2019art}USENIX'19} & \rot[90]{\cite{qin2022quantifying}SSP'22} & \rot[90]{\cite{zhou2021high}SSP'21} & \rot[90]{\cite{cecchetti2021compositional}SSP'21} & \rot[90]{\cite{daian2020flash}SSP'20} & \rot[90]{\cite{jiao2020semantic}SSP'20} & \rot[90]{\cite{zhang2019lay}SSP'19} & \rot[90]{\cite{saad2021revisiting}CCS'21} & \rot[90]{\cite{lewis2021does}CCS'21} & \rot[90]{\cite{das2021exact}CCS'21} & \rot[90]{\cite{li2021deter}CCS'21} & \rot[90]{\cite{saad2021syncattack}CCS'21} & \rot[90]{\cite{mirkin2020bdos}CCS'20} & \rot[90]{\cite{chen2019tokenscope}CCS'19} & \rot[90]{\cite{das2019formal}CCS'19} & \rot[90]{\cite{tsabary2018gap}CCS'18} & \rot[90]{\cite{kiffer2018better}CCS'18} & \rot[90]{\cite{li2021strong}NDSS'21} & \rot[90]{\cite{bissias2020bobtail}NDSS'20} & \rot[90]{\cite{perez2019broken}NDSS'20} & \rot[90]{\cite{wan2021smart}ICSE'21} & \rot[90]{\cite{durieux2020empirical}ICSE'20} & \rot[90]{\cite{hwang2020gap}ICSE'20} & \rot[90]{\cite{liu2021characterizing}ASE'21} & \rot[90]{\cite{xue2020cross}ASE'20} & \rot[90]{\cite{grossman2017online}POPL'18} & \rot[90]{\cite{li2020securing}PLDI'20} & \rot[90]{\cite{brent2020ethainter}PLDI'20} & \rot[90]{\cite{beillahi2020behavioral}PLDI'20} & \rot[90]{\cite{gervais2016security}} & \rot[90]{\cite{wust2016ethereum}} & \rot[90]{\cite{marcus2018low}} & \rot[90]{\cite{mirkin2020bdos}} & \rot[90]{\cite{rahimian2021tokenhook}} & \rot[90]{\cite{gudgeon2020decentralized}} & \rot[90]{\cite{guarnizo2019pdfs}} & \rot[90]{\cite{breidenbach2021chainlink}} & \rot[90]{\cite{qin2021attacking}} & \rot[90]{\cite{beosin2021wakaswap}} & \rot[90]{\cite{boesin2021sato}} & \rot[90]{\cite{boesin2021pinecone}} & \rot[90]{\cite{boesin2021ctoken}} & \rot[90]{\cite{boesin2021beatsquare}} & \rot[90]{\cite{peckshield2021rabbit}} & \rot[90]{\cite{peckshield2021Hegic}} & \rot[90]{\cite{peckshield2021DeriV2}} & \rot[90]{\cite{peckshield2021Coin98}} & \rot[90]{\cite{peckshield2021AngryMining}} & \rot[90]{\cite{slowmist2021jswap}} & \rot[90]{\cite{slowmist2021supremex}} & \rot[90]{\cite{slowmist2021solyard}} & \rot[90]{\cite{slowmist2021cookfinance}} & \rot[90]{\cite{consensys2021defisaver}} & \rot[90]{\cite{consensys2021fei}} & \rot[90]{\cite{consensys2021gitcoin}} & \rot[90]{\cite{consensys2021wheat}} & \rot[90]{\cite{consensys2021umbra}} & \rot[90]{\cite{certik2021Zoo}} & \rot[90]{\cite{certik2021Trister}} & \rot[90]{\cite{certik2021Rezerve}} & \rot[90]{\cite{certik2021LFW}} & \rot[90]{\cite{certik2021gamedao}} & \rot[90]{\cite{trailofbits2021complifi}} & \rot[90]{\cite{trailofbits2021frax}} & \rot[90]{\cite{trailofbits2021yearn}} & \rot[90]{\cite{openzeppelin2021cLabs}} & \rot[90]{\cite{openzeppelin2021celo}} & \rot[90]{\cite{openzeppelin2021fei}} &  &  & \\
\multirow{9}{*}{\rot[90]{\textbf{Network}}} & Network layer transparency / privacy & \clg{Transaction content transparency} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{5} & \clg{}\\
 &  & Propagation transparency &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 3 & \\
 & Improper peer discovery / churning logic & \clg{Eclipse} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{7} & \clg{}\\
 &  & Sybilattack &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} &  & \\
 & Network congestion & \clg{Intentional DoS} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{1} & \clg{4} & \clg{}\\
 &  & Unintentional DoS &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{1} &  & \\
 & Exposed internet service & \clg{Sensitive DNS servers} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{2} & \clg{3} & \clg{}\\
 &  & Unreliable BGP messages &  & \ding{108} & \ding{108} & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 3 & \\
 & Other network vulnerabilities & \clg{-} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{1} & \clg{}\\
\midrule
\multirow{11}{*}{\rot[90]{\textbf{Consensus}}} & Blockchain protocol vulnerabilities & - &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} &  & \\
 & Unstable / greedy incentive mechanism & \clg{Majority / 51\% attack} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{5} & \clg{}\\
 &  & Block reorganization &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 2 & \\
 &  & \clg{Selfish mining} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{7} & \clg{}\\
 &  & Double spending &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  & \ding{108} &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 6 & \\
 &  & \clg{Feather forking} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{2} & \clg{}\\
 &  & Bribery attacks &  & \ding{108} &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 2 & \\
 &  & \clg{Other incentive-based incidents} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{6} & \clg{}\\
 & Unfair sequencing & Sequencer transaction order manipulation &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 2 & \\
 &  & \clg{Transaction censoring} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{1} & \clg{}\\
 & Other consensus vulnerabilities & - &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 3 & \\
\midrule
\multirow{17}{*}{\rot[90]{\textbf{Smart Contract}}} & State transition design / implementation & \clg{Under-priced opcodes} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{2} & \clg{}\\
 &  & Outdated compiler version &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  &  &  & & \cellcolor{r0}{} &  & 11\\
 & Untrusted callee / race condition & \clg{Direct call to untrusted contract} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{4} & \clg{3} & \clg{16}\\
 &  & Reentrancy & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} &  & \ding{108} &  & \ding{108} & \ding{108} &  &  & \ding{108} &  &  &  & \ding{108} & \ding{108} & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  &  &  & \ding{108} & \ding{108} &  &  &  &  &  & \ding{108} &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  & \ding{109} &  & \ding{109} &  &  &  &  &  &  &  &  &  & & \cellcolor{r2}{12} & 31 & 16\\
 &  & \clg{Delegatecall / call injection} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{2} & \clg{13} & \clg{8}\\
 & Coding mistake & Unhandled or mishandled exception & \ding{108} &  &  & \ding{108} &  & \ding{108} &  & \ding{108} & \ding{108} &  &  &  &  &  &  & \ding{108} &  &  & \ding{108} & \ding{108} &  &  &  & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  &  &  &  & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  & \ding{108} &  &  &  & \ding{108} &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  & & \cellcolor{r0}{} & 22 & 2\\
 &  & \clg{Locked or frozen asset} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{1} & \clg{11} & \clg{2}\\
 &  & Integer overflow or underflow & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} &  & \ding{108} &  &  &  &  & \ding{108} & \ding{108} & \ding{108} &  &  &  &  &  &  & \ding{108} & \ding{108} & \ding{108} & \ding{108} & \ding{108} &  &  & \ding{108} &  &  &  &  &  & \ding{108} & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  &  &  &  &  &  &  & \ding{109} & \ding{109} &  &  & & \cellcolor{r0}{} & 21 & 16\\
 &  & \clg{Absence of coding logic or sanity check} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}}& \cellcolor{r10}{44} & \clg{9} & \clg{12}\\
 &  & Short address &  &  & \ding{108} & \ding{108} &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 4 & 4\\
 &  & \clg{Casting} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{4} & \clg{1}\\
 &  & Unbounded or gas costly operation & \ding{108} &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  & \ding{108} &  &  &  &  & \ding{108} & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  & & \cellcolor{r0}{} & 7 & 1\\
 &  & \clg{Arithmetic mistakes} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{\ding{109}}& \cellcolor{r0}{2} & \clg{4} & \clg{23}\\
 &  & Other coding mistakes & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  & \ding{108} &  &  &  &  & \ding{108} &  & \ding{108} & \ding{108} &  &  &  & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} & \ding{109} & \ding{109} & \ding{109} &  & \ding{109} & \ding{109} & \ding{109} & \ding{109} & \ding{109} & \ding{109} & & \cellcolor{r1}{6} & 8 & 11\\
 & Access control & \clg{Inconsistent access control} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{}& \cellcolor{r1}{5} & \clg{14} & \clg{18}\\
 &  & Visibility error, including unrestricted action & \ding{108} &  &  & \ding{108} &  & \ding{108} &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  & \ding{108} &  & \ding{108} &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  & & \cellcolor{r1}{6} & 9 & 15\\
 & Other smart contract vulnerabilities & \clg{-} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{\ding{109}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{\ding{109}} & \clg{} & \clg{\ding{109}} & \clg{\ding{109}}& \cellcolor{r0}{1} & \clg{20} & \clg{22}\\
\midrule
\multirow{20}{*}{\rot[90]{\textbf{Protocol}}} & Transaction order dependency & Front-running &  & \ding{108} &  & \ding{108} & \ding{108} &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  & \ding{108} &  &  &  & \ding{108} &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  & \ding{108} &  &  & \ding{108} &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} &  &  &  & \ding{109} &  &  &  &  &  &  & \ding{109} &  & \ding{109} &  &  & & \cellcolor{r0}{2} & 12 & 17\\
 &  & \clg{Back-running} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{\ding{111}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{7} & \clg{14}\\
 &  & Sandwiching &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  & \ding{108} & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} & \ding{111} &  &  &  & \ding{109} &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 4 & 15\\
 &  & \clg{Other transaction order dependency} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{3} & \clg{}\\
 & Replayable design & Transaction / strategy replay &  &  & \ding{108} & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 2 & 9\\
 & Block state dependency & \clg{Randomness} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{6} & \clg{5}\\
 &  & Other block state dependency & \ding{108} &  &  & \ding{108} &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  & \ding{108} & \ding{108} &  & \ding{108} & \ding{108} & \ding{108} &  & \ding{108} &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} & \ding{109} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 13 & 2\\
 & Fake contracts & \clg{Fake token} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r2}{9} & \clg{1} & \clg{}\\
 &  & Other fake contracts &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{1} &  & \\
 & Unsafe DeFi protocol dependency & \clg{On-chain oracle manipulation} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r6}{28} & \clg{4} & \clg{}\\
 &  & Governance attack &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{3} & 2 & \\
 &  & \clg{Token standard incompatibility} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r2}{9} & \clg{2} & \clg{}\\
 &  & Flash liquidity borrow, purchase, mint or deposit &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r2}{9} & 2 & \\
 &  & \clg{Unsafe call to phantom function} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{1} & \clg{} & \clg{}\\
 &  & Other unsafe DeFi protocol dependency &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r1}{7} &  & 1\\
 & Unsafe DeFi protocol interaction & \clg{Unfair slippage protection} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{3} & \clg{3} & \clg{}\\
 &  & Unfair liquidity providing &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{4} &  & 1\\
 &  & \clg{Unsafe or infinite token approval} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{} & \clg{}\\
 &  & Other unfair or unsafe DeFi protocol interaction &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{109} &  &  & \ding{109} &  &  &  & & \cellcolor{r0}{1} & 1 & 2\\
 & Other protocol vulnerabilities & \clg{-} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{3} & \clg{1} & \clg{}\\
\midrule
\multirow{14}{*}{\rot[90]{\textbf{Auxilary Services}}} & Faulty web development & - &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{1} &  & \\
 & Faulty operation & \clg{Compromised private key / wallet} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r5}{22} & \clg{3} & \clg{}\\
 &  & Weak password &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 1 & \\
 &  & \clg{Deployment mistake} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{\ding{110}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r1}{6} & \clg{} & \clg{5}\\
 & Off-chain oracle manipulation & Malicious oracle updater &  & \ding{108} &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} & \ding{108} &  &  &  &  &  &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 4 & 5\\
 &  & \clg{Malicious data source} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{4} & \clg{}\\
 &  & External market manipulation &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 1 & \\
 & Greedy & \clg{Backdoor / Honeypot} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{\ding{108}} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r2}{10} & \clg{3} & \clg{}\\
 &  & Insider trade or other activities &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{3} & 1 & \\
 &  & \clg{Phishing attack} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{2} & \clg{} & \clg{}\\
 &  & Authority control or breach of promise &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{110} & \ding{110} &  & \ding{110} & \ding{110} & \ding{110} & \ding{110} & \ding{110} &  &  &  &  &  & \ding{109} & \ding{109} & \ding{109} & \ding{109} & \ding{109} &  &  &  &  &  & & \cellcolor{r2}{13} & 1 & 12\\
 & Faulty blockchain service provider & \clg{Faulty wallet provider} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{} & \clg{} & \clg{}\\
 &  & Faulty API / RPC &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \ding{108} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & \cellcolor{r0}{} & 2 & \\
 & Other Auxilary service vulnerabilities & \clg{-} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{} & \clg{}& \cellcolor{r0}{2} & \clg{} & \clg{}\\

\bottomrule
\end{tabular}
}
\end{table}
\end{landscape}
}
